The Chemo-Dynamical Groups of Galactic Globular Clusters

We introduce a multi-component chemo-dynamical method for splitting the Galactic population of Globular Clusters (GCs) into three distinct constituents: bulge, disc, and stellar halo. The latter is further decomposed into the individual large accretion events that built up the Galactic stellar halo: the Gaia-Enceladus-Sausage, Kraken and Sequoia structures, and the Sagittarius and Helmi streams. Our modelling is extensively tested using mock GC samples constructed from the AURIGA suite of hydrodynamical simulations of Milky Way (MW)-like galaxies. We find that, on average, a proportion of the accreted GCs cannot be associated with their true infall group and are left ungrouped, biasing our recovered population numbers to approximately 80 percent of their true value. Furthermore, the identified groups have a completeness and a purity of only 65 percent. This reflects the difficulty of the problem, a result of the large degree of overlap in energy-action space of the debris from past accretion events. We apply the method to the Galactic data to infer, in a statistically robust and easily quantifiable way, the GCs associated with each MW accretion event. The resulting groups' population numbers of GCs, corrected for biases, are then used to infer the halo and stellar masses of the now defunct satellites that built up the halo of the MW.

==> Original4.2.tex <==

\subsection{Testing on Mock Samples}

We now apply our method to the relaxed \auriga{} sample, with each halo having $1000$ mock realisations.
To quantify how well the method performs across our samples we calculate the following quantities.
For a group with true GC count, \Ntrue, that the fit predicts to contain \Nfit{} members, 
and their intersection $N_{\cap}$, we define the purity, $P$, and completeness, $C$, of the fit as:
\begin{align}\label{Eq:Scoring}
     P &= N_{\cap} / N_{\mathrm{fit}}\\
     C &= N_{\cap} / N_{\mathrm{true}}.
\end{align}


\begin{figure}
	\includegraphics[width=\columnwidth]{Plots/Ntrue_Nfit_Frac_ax.pdf}
	\smallspace{}
	\caption{
	The true group population, $N_{\mathrm{true}}$, against the fit group population, $N_{\mathrm{fit}}$,
	as a fraction of $N_{\mathrm{true}}$ for our mock GC sample.
	We bin the accreted groups
	\Change{(not including the ungrouped component)}
	in $N_{\mathrm{true}}$, and, using a Gaussian smoothing kernel of $\sigma=2$,
	show the median and $16\%-84\%$ range with shaded regions for the distribution of $N_{\mathrm{fit}}$ (green).
	The symbols with error bars show the individual in-situ components, the total in-situ sample, and the ungrouped components.
	Note that the disc and bulge components of the mocks have populations of 20 and 40 by construction,
	whereas the population of the ungrouped component depends upon the accretion history of the halo.
	}
	\label{fig:Mock_NtrueNfit}
\end{figure}

\begin{figure}
	\includegraphics[width=1\columnwidth]{Plots/Ntrue_PurityCompletness_ax.pdf}
	\smallspace{}
	\caption{
	The true group population, $N_{\mathrm{true}}$, against the purity, $P$ (top panel),
	and completeness, $C$ (bottom panel), of our fitted mock GC sample (see main text for definitions).
	We bin the results for the accreted groups in $N_{\mathrm{true}}$,
	using a Gaussian smoothing kernel of $\sigma=2$,
	and show the median and $16\%-84\%$ range
	with the shaded regions for the distribution of $N_{\mathrm{fit}}$.
	The symbols with error bars show the individual bulge and disc components, total in-situ sample, and ungrouped component.
	}
	\label{fig:Mock_NtruePurityComp}
\end{figure}


First, we consider the true group population against the fit populations in Fig.~\ref{fig:Mock_NtrueNfit}.
Across the total sample, we recover the accreted population numbers with an under-bias of $\sim10\%$,
with a somewhat large group-to-group variance of $\sim50\%$ for the smallest groupings.
These `missing clusters' corresponding to the $\sim10\%$ bias can be found in the ungrouped component, which is systematically too large by $\sim30\%$.
However, there are clear trends if we look at the results as a function of the size of the group.

For smaller groups ($\lessapprox 15$) there is significant fractional scatter as the changing membership of
a single cluster corresponds to a larger proportion of the group.
The smallest groups can be seen to have a small chance of disappearing (their population dropping to zero),
which can happen when the group is too spread out to be reliably identified.
We find that we systematically underestimate the population of the larger groups ($\gtrsim10$),
although the scatter in the relation is significantly reduced compared to that for the smaller groups.

These trends continue if we consider the purity and completeness of our fits against the true group population
-- see Fig.~\ref{fig:Mock_NtruePurityComp}.
\Change{We find that, on average, for all groups we achieve a purity and a completeness of $\sim67\%$.
For the accreted groups, we find a purity of $\sim64\%$ and a completeness of $\sim55\%$.}
There are no clear trends in the purity against the true population number.
However, there is a clear decrease in the completeness of the groups as the true population increases.

These trends are likely a reflection of the mass of the corresponding accretion event and its effect on
the corresponding group's distribution in phase space.
The larger groups have greater spread in phase space due to their higher internal velocity dispersion before accretion
and tend to exist at lower energies because they experience greater dynamical friction.
These factors directly impact our ability to recover the groups.
Due to the wider spread in the dynamical space, and the crowded nature of the lower energy regions,
more of the GCs are misattributed to other groups.
The smaller groups tend to be more densely distributed in phase space, and typically exist at higher energies
(unless accreted at early times).
Providing the group itself has enough members to be reliably identified, they are recovered with greater confidence.

As already noted, the average population of the ungrouped component increases by the addition of GCs that
could not be identified within their groups.
These are typically separated from the rest of their accreted group in phase space,
where they are difficult to identify, and so they fall into the ungrouped component.
This is also reflected in the low purity of this component, whilst the completeness is marginally better,
suggesting that ungrouped GCs are not normally being misattributed to other structures.

The total in-situ population is, in general, well recovered with very high purity.
Rarely does the methodology misidentify an accreted GC as an in-situ one in our mock tests,
with a median purity of $98\%$.
Compared to most of the accreted components, the in-situ components occupy distinct positions in the chemo-dynamical space.
Groups that do overlap with the in-situ populations tend to be older and
larger mergers that can bring their material to the heart of the galaxy.
For the individual components, the performance is marginally worse, notably for the bulge GCs.
Because of the overlap between the individual components, there is some reshuffling between the bulge and disc groups.

